LMM4LMM: Benchmarking and Evaluating Large-multimodal Image Generation with LMMs

Recent breakthroughs in large multimodal models (LMMs) have significantly advanced both text-to-image (T2I) generation and image-to-text (I2T) interpretation. However, many generated images still suffer from issues related to perceptual quality and text-image alignment. Given the high cost and inefficiency of manual evaluation, an automatic metric that aligns with human preferences is desirable. To this end, we present EvalMi-50K, a comprehensive dataset and benchmark for evaluating large-multimodal image generation, which features (i) comprehensive tasks, encompassing 2,100 extensive prompts across 20 fine-grained task dimensions, and (ii) large-scale human-preference annotations, including 100K mean-opinion scores (MOSs) and 50K question-answering (QA) pairs annotated on 50,400 images generated from 24 T2I models. Based on EvalMi-50K, we propose LMM4LMM, an LMM-based metric for evaluating large multimodal T2I generation from multiple dimensions including perception, text-image correspondence, and task-specific accuracy. Extensive experimental results show that LMM4LMM achieves state-of-the-art performance on EvalMi-50K, and exhibits strong generalization ability on other AI-generated image evaluation benchmark datasets, manifesting the generality of both the EvalMi-50K dataset and LMM4LMM metric. Both EvalMi-50K and LMM4LMM will be released at https://github.com/IntMeGroup/LMM4LMM.

==> tabels/SRCC_ACC_ORI.tex <==
\begin{table*}[tbph]
\vspace{-5mm}
\setlength{\belowcaptionskip}{-0.01cm}
\centering
\belowrulesep=0pt
\aboverulesep=0pt
\renewcommand\arraystretch{0.87}
\caption{Performance comparisons of LMMs on the EvalMi-50K. We report SRCC of quality MOS ($\text{SRCC}_q$), correspondence MOS ($\text{SRCC}_c$), and QA accuracy (Acc). 
The best results are marked in {\textcolor{red}{RED}} and the second-best in {\blue{BLUE}}. 
*refers to finetuned scores.
}
\vspace{-3mm}
   \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c|cc:c|cc:c}
    \toprule[1pt]
     %\midrule
     Dimension  &\multicolumn{3}{c}{\textbf{Single Object}}&\multicolumn{3}{c}{\textbf{Two Objects}}&\multicolumn{3}{c}{\textbf{Counting}}&\multicolumn{3}{c}{\textbf{Colors}}&\multicolumn{3}{c}{\textbf{Position}}&\multicolumn{3}{c}{\textbf{Shapes}}&\multicolumn{3}{c}{\textbf{Texture}}\\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}\cmidrule(lr){20-22}
 Methods / Metrics
&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$\\
    \midrule
     LLaVA-1.5 (7B)~\cite{liu2024improved} & 0.2950  & 0.2321 & 0.8415 & 0.3707  & 0.5441 & 0.7810 & 0.1299 & 0.3874 & 0.6136 & 0.3019  & 0.3219 & 0.8491 & 0.3724 & 0.4739 & 0.4569 & 0.3573 & 0.1829 & 0.5323 & 0.1904 & 0.2150 & 0.6384  \\
    LLaVA-NeXT (8B)~\cite{liu2024llavanext} & 0.3931 & 0.2439  & 0.8345 & 0.4588 & 0.4505 & 0.7905 & 0.3189 & 0.4600 & 0.6841 & 0.3082 & 0.4240 & 0.8350 & 0.4336 & 0.4082  & 0.4625 & 0.4030 & 0.4326 & 0.5970 & 0.3684 & 0.4943 & 0.6272  \\
    mPLUG-Owl3 (7B)~\cite{ye2024mplug} & 0.4674 & 0.2375  & 0.8508 & 0.4295 & 0.5261 & 0.8114 & 0.4326 & 0.5814 & 0.8227 & 0.4488 & 0.3602 & 0.8431 & 0.4257 & 0.4982  & 0.5243 & 0.4140 & 0.3199 & 0.5796 & 0.4000 & 0.2888 & 0.6763 \\ 
   MiniCPM-V2.6 (8B)~\cite{yao2024minicpm}& 0.4230 & 0.3503  & 0.8508 & 0.3114 & 0.6965 & 0.7790 & 0.3614 & 0.7106 & 0.8386 & 0.3534 & 0.5471 & 0.8551 & 0.4445 & 0.6074  & 0.5562 & 0.4515 & 0.5332 & 0.6915 & 0.3014 & 0.5449 & 0.7455\\
    Qwen2-VL (7B)~\cite{Qwen2-VL} & 0.4249 & 0.1632  & 0.8438 & 0.2004 & 0.6726 & 0.7905 & 0.3143 & 0.6967 & 0.7818 & 0.3571 & 0.4413 & 0.8410 & 0.2238 & 0.5522  & 0.5974 & 0.2646 & 0.4996 & 0.5896 & 0.2341 & 0.4051 & 0.6607\\
     Qwen2.5-VL(7B)~\cite{Qwen2.5-VL}& 0.5068  & 0.3941 & 0.8508 & 0.4950  & 0.7158 & 0.8210 & 0.4926 & 0.7051 & 0.8545 & 0.5236  & 0.5047 & 0.8712 & 0.5685 & 0.6479 & 0.8071 & 0.6024 & 0.4843 & 0.6592 & 0.4264 & 0.5923 & 0.7679\\
    Llama3.2-Vision (11B)~\cite{meta2024llama}
    &0.2648&0.2753&0.8508&0.1968&0.1851&0.7366&0.4021&0.2842&0.7364&0.2125&0.3162 &0.8793&0.2330&0.15375&0.4894&0.2515&0.3011&0.6658&0.2570&0.3594&0.7232\\
    DeepseekVL (7B)~\cite{lu2024deepseekvl}
    &0.1367&0.0433&0.8251&0.1919&0.4470&0.7410&0.2216&0.1940&0.7886&0.0942&0.1338&0.8028&0.2750&0.3318&0.5974&0.2127&0.0300&0.6119&0.1110&0.1004&0.7165 \\
    DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.1404 &0.0322 &0.7837 &0.1566 &0.0512 &0.7278 &0.0351 &0.0282&0.8170 &0.0699 &0.0461 &0.8001 &0.0482 &0.0494 &0.7018 &0.1358 &0.0352 &0.7929 &0.0775 &0.0380 &0.7929\\
    DeepseekVL2 (2B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.1875 &0.0224 &0.4406 &0.2191 &0.0916 &0.4495 &0.2312 &0.0164&0.5545 &0.1640 &0.0824 &0.3260 &0.1701 &0.0555 &0.4757 &0.3304 &0.0453 &0.5050 & 0.2160 & 0.0549 & 0.5781\\
  CogAgent (18B)~\cite{hong2024cogagentvisuallanguagemodel}& 0.3411 & 0.3162  & 0.8531 & 0.2915 & 0.5355 & 0.8133 & 0.3191 & 0.3890 & 0.7114 & 0.4329 & 0.3783 & 0.8431 & 0.4074 & 0.4101  & 0.3521 & 0.4916 & 0.3172 & 0.5746 & 0.3089 & 0.3025 & 0.6228 \\
  InternVL2 (8B)~\cite{wang2024mpo}& 0.1230 & 0.3695  & 0.8345 & 0.1447 & 0.6436 & 0.8229 & 0.0701 & 0.5815 & 0.7136 & 0.0890 & 0.5478 & 0.8652 & 0.1585 & 0.6041  & 0.5412 & 0.0982 & 0.4042 & 0.6393 & 0.1226 & 0.5715 & 0.7232\\
    InternVL2.5 (8B)~\cite{chen2024expanding}& 0.2334  & 0.2245 & 0.8345 & 0.2533  & 0.6250 & 0.7905 & 0.2045 & 0.5740 & 0.7159 & 0.1846  & 0.3552 & 0.8390 & 0.3062 & 0.5653 & 0.5618 & 0.1972 & 0.4360 & 0.5846 & 0.1615 & 0.4972 & 0.6964 \\
   InternLM-XComposer (7B)~\cite{internlmxcomposer}& 0.4674 & 0.1372  & 0.8508 & 0.4295 & 0.1338 & 0.8114 & 0.4326 & 0.3370 & 0.8227 & 0.4488 & 0.1519 & 0.8431 & 0.4257 & 0.2045  & 0.5243 & 0.4140 & 0.0388 & 0.5796 & 0.4000 & 0.0312 & 0.6763\\
    Llava-Onevision (0.5B)~\cite{li2024llava}& 0.1099 & 0.2670 & 0.7692 & 0.0068 & 0.3457 & 0.6057 & 0.0605 & 0.2331 & 0.7591 & 0.0460 & 0.1960 & 0.8571 & 0.0865 & 0.1988 & 0.7228 & 0.2047 & 0.2224 & 0.5871 & 0.0685 & 0.2074 & 0.6808\\
   \hline
   *DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&\bf\blue{0.7719} & \bf\blue{0.6581}& 0.8914 &\bf\blue{0.7841} &0.8250 &0.8781 &\bf\blue{0.7656} &\bf\blue{0.8200}& 0.8691 &\bf\blue{0.7744} & \bf\blue{0.7505} &\bf\blue{0.8945} &\bf\blue{0.7947} & 0.6043 & 0.8475&\bf\blue{0.7989}  &0.6043& 0.7687&\bf\blue{0.7381} &0.7013& 0.8147\\
   *Qwen2.5-VL (8B)~\cite{Qwen2.5-VL}& 0.7076  & 0.6090 & \bf\blue{0.8950} & 0.7046  & \bf\blue{0.8280} & \bf\blue{0.8922} & 0.6993& 0.7631 & \bf\blue{0.8743} & 0.6805  & 0.6606 & 0.8915 & 0.6895& \bf\blue{0.7768} & \bf\blue{0.8826} & 0.7246 & \bf\blue{0.7881} & \bf\blue{0.8159} & 0.5848 & \bf\blue{0.7879} & \bf\blue{0.8616}\\
   *Llama3.2-Vision (11B)~\cite{meta2024llama}&0.7056 & 0.5577& 0.8415& 0.7344& 0.6134& 0.7257&0.7294 &0.5102&0.6614&0.7228 & 0.4597& 0.8089&0.7469 & 0.3569& 0.7790&0.7324 & 0.5184&0.7015&0.7107 & 0.5702&0.7009\\
   
   \rowcolor{gray!20} \textbf{LMM4LMM (Ours)} &\bf\red{0.8497}&\bf{\red{0.7989}}&\bf\red{0.8951}&\bf\red{0.8608}&\bf\red{0.8989}&\bf\red{0.8933}&\bf\red{0.8681}&\bf\red{0.8667}&\bf\red{0.8750}&\bf\red{0.8597}&\bf\red{0.8260}&\bf\red{0.8954}&\bf\red{0.8512}&\bf\red{0.8411}&\bf\red{0.8876}&\bf\red{0.8627}&\bf\red{0.8167}&\bf\red{0.8184}&\bf\red{0.8053}&\bf\red{0.8522}&\bf\red{0.8705}\\
   %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
    \bottomrule[1pt]
  \end{tabular}}
    \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c|cc:c|cc:c}
    \toprule[1pt]
     %\midrule
     Dimension  &\multicolumn{3}{c}{\textbf{Scene}}&\multicolumn{3}{c}{\textbf{Style}}&\multicolumn{3}{c}{\textbf{OCR}}&\multicolumn{3}{c}{\textbf{HOI}}&\multicolumn{3}{c}{\textbf{Human}}&\multicolumn{3}{c}{\textbf{Emotion}}&\multicolumn{3}{c}{\textbf{Linguistic Structure}}\\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}\cmidrule(lr){20-22}
 Methods / Metrics
&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$\\
    \midrule
     LLaVA-1.5(7B)~\cite{liu2024improved}& 0.3371  & 0.2976 & 0.9221 & 0.4448  & 0.2088 & 0.7397 & 0.4540 & 0.6660 & 0.8341 & 0.4570  & 0.4278 & 0.7182 & 0.4474 & 0.4283 & 0.8385 & 0.2875 & 0.4226 & 0.6342 & 0.4268 & 0.2776 & 0.7716 \\
    LLaVA-NeXT(8B)~\cite{liu2024llavanext}& 0.5165 & 0.3357  & 0.8734 & 0.5022 & 0.3259 & 0.7763 & 0.5603 & 0.6294 & 0.9258 & 0.5213 & 0.5959 & 0.7581 & 0.4856 & 0.3101  & 0.8530 & 0.4436 & 0.5017 & 0.5586 & 0.5652 & 0.5646 & 0.8065 \\
    mPLUG-Owl3(7B)~\cite{ye2024mplug}& 0.4482 & 0.0128 & 0.8734 & 0.2093 & 0.2021 & 0.7671 & 0.3605 & 0.6685 & 0.8603 & 0.4603 & 0.4978 & 0.7531 & 0.4602 & 0.4434  & 0.8323 & 0.3333 & 0.5003 & 0.6288 & 0.4989 & 0.5554 & 0.8462 \\ 
       MiniCPM-V2.6(8B)~\cite{yao2024minicpm}& 0.3687 & 0.1263  & 0.8734 & 0.4749 & 0.4674 & 0.7763 & 0.5249 & 0.7265 & 0.8559 & 0.4026 & 0.5450 & 0.7456 & 0.4497 & 0.4777  & 0.8571 & 0.3133 & 0.5152 & 0.6414 & 0.4358 & 0.6568 & 0.8252\\
    Qwen2-VL(7B)~\cite{Qwen2-VL}& 0.3980 & 0.2974  & 0.8766 & 0.5250 & 0.4392 & 0.7557 & 0.5110 & 0.7198 & 0.9214 & 0.2926 & 0.5666 & 0.7506 & 0.2501 & 0.5739  & 0.8261 & 0.4171 & 0.5737 & 0.6234 & 0.4853 & 0.6932 & 0.8252\\
     Qwen2.5-VL(7B)~\cite{Qwen2.5-VL}& 0.5478  & 0.4350 & 0.9188 & 0.5374  & 0.4236 & 0.7443 & 0.6581 & 0.7734 & 0.9039 & 0.5189  & 0.5432 & 0.7706 & 0.5603 & 0.4540 & 0.8012 & 0.4405 & 0.4930 & 0.5099 & 0.6096 & 0.7007 & 0.8438\\
    Llama3.2-Vision(11B)~\cite{meta2024llama}
    &0.3547&0.0472&0.9218&0.4085&0.3423&0.7506&0.1781&0.2582&0.8879&0.2769&0.0856 &0.7232&0.1960&0.1615&0.6921& 0.2374& 0.1284& 0.5903& 0.3215 &0.4415 &0.5903\\
    DeepseekVL (7B)~\cite{lu2024deepseekvl}
    &0.3330&0.1092&0.8896&0.3005&0.0123&0.7580&0.3515&0.1990&0.7424&0.3598&0.2861&0.7032&0.4564&0.1408&0.7847&0.2493&0.3299&0.6595&0.4436&0.5019&0.8392 \\ 
    DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.1404 &0.5673 &0.1566 &0.1566 &0.0351 &0.7278 &0.0699 &0.6081&0.0482 &0.0482 &0.1358 &0.8001 &0.1358 &0.5355 &0.7018 &0.0775 &0.5825 &0.7929&0.2565 &0.0133 &0.7646\\
    DeepseekVL2 (2B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.3410 &0.0226 &0.7175 &0.3403 &0.0464 &0.5457 &0.4329 &0.1551 &0.2620 &0.3279 &0.0198 &0.4938 &0.2298 &0.0187 &0.7246 &0.1676 &0.0112 &0.3568 & 0.4062 & 0.0420 & 0.5897\\
  CogAgent(18B)~\cite{hong2024cogagentvisuallanguagemodel}& 0.3565 & 0.0241  & 0.8734 & 0.5862 & 0.2524 & 0.7740 & 0.4927 & 0.3833 & 0.6507 & 0.4597 & 0.3074 & 0.7157 & 0.3556 & 0.1628  & 0.8033 & 0.2977 & 0.2560 & 0.6162 & 0.4823 & 0.4043 & 0.8298 \\
    InternVL2(8B)~\cite{wang2024mpo} & 0.1899 & 0.1946  & 0.8734 & 0.4383 & 0.5235 & 0.7237 & 0.2537 & 0.6595 & 0.8515 & 0.2062 & 0.4766 & 0.7506 & 0.0633 & 0.4308  & 0.8613 & 0.1378 & 0.4761 & 0.5117 & 0.3134 & 0.6197 & 0.8042\\
    InternVL2.5(8B)~\cite{chen2024expanding}& 0.2177  & 0.2160 & 0.8994 & 0.3435  & 0.4061 & 0.7443 & 0.3487 & 0.6659 & 0.7205 & 0.3546  & 0.4728 & 0.7357 & 0.2490 & 0.4458 & 0.8199 & 0.2366 & 0.5174 & 0.5820 & 0.3566 & 0.6126 & 0.7459 \\
   InternLM-XComposer(7B)~\cite{internlmxcomposer}& 0.4482 & -0.0034 & 0.8734 & 0.2093 & 0.0264 & 0.7671 & 0.3605 & 0.0599 & 0.8603 & 0.4603 & 0.2748 & 0.7531 & 0.4602 & 0.0797  & 0.8323 & 0.3333 & 0.1571 & 0.6288 & 0.4989 & 0.3460 & 0.8462\\
    Llava-Onevision(0.5B)~\cite{li2024llava}& 0.1844 & 0.3412 & 0.8766 & 0.2037  & 0.3358 & 0.6164 & 0.2900 & 0.0586 & 0.7598 & 0.0210 & 0.2987 & 0.5636 & 0.0430 & 0.3270 & 0.2153 & 0.1076 & 0.3139 & 0.6270 & 0.1655 & 0.0327 & 0.7646\\
   \hline
   *DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&\bf\blue{0.7628} & \bf\blue{0.5913}& 0.9318 &\bf\blue{0.7297} &\bf\blue{0.6765} & \bf\blue{0.8379} &0.8552 &0.8247& 0.9120 &\bf\blue{0.7999} & \bf\blue{0.6665} & 0.8030 &\bf\blue{0.8456} & \bf\blue{0.7188} & 0.8841 &\bf\blue{0.7902}  &0.6695& 0.7982 &\bf\blue{0.8124} &0.3752& 0.8718\\
   *Qwen2.5-VL (8B)~\cite{Qwen2.5-VL}& 0.6795  & 0.5212 & \bf\blue{0.9321} & 0.6683  & 0.6424 & 0.8365 & \bf\blue{0.8810}& \bf\blue{0.8498} & \bf\blue{0.9294} & 0.7509  & 0.6107 & \bf\blue{0.8354} & 0.6929& 0.5616 & \bf\blue{0.9196} & 0.6333 & \bf\blue{0.6899} & \bf\blue{0.8288} & 0.7540 & \bf\blue{0.7951} & \bf\blue{0.8834}\\
    *Llama3.2-Vision (11B)~\cite{meta2024llama}&0.7601 & 0.4558& 0.9253& 0.7195& 0.4814& 0.7900&0.8416 &0.5261&0.8035&0.7902 & 0.4693& 0.7456&0.8165 & 0.6347& 0.8447&0.7548 & 0.4625&0.7748&0.8007& 0.2726&0.7366\\
   %\hdashline
   \rowcolor{gray!20} \textbf{LMM4LMM (Ours)} &\bf\red{0.8563}&\bf{\red{0.7554}}&\bf\red{0.9323}&\bf\red{0.8597}&\bf\red{0.8042}&\bf\red{0.8607}&\bf\red{0.9383}&\bf\red{0.8815}&\bf\red{0.9301}&\bf\red{0.9205}&\bf\red{0.8642}&\bf\red{0.8304}&\bf\red{0.9156}&\bf\red{0.8514}&\bf\red{0.9199}&\bf\red{0.9065}&\bf\red{0.8642}&\bf\red{0.8468}&\bf\red{0.8778}&\bf\red{0.8374}&\bf\red{0.8841}\\
   %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
    \bottomrule[1pt]
  \end{tabular}}
      \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:c|cc:c|cc:c|cc:c|cc:c|cc:c|cc:c}
    \toprule[1pt]
     %\midrule
     Dimension  &\multicolumn{3}{c}{\textbf{View}}&\multicolumn{3}{c}{\textbf{Knowledge}}&\multicolumn{3}{c}{\textbf{Face}}&\multicolumn{3}{c}{\textbf{Imagination}}&\multicolumn{3}{c}{\textbf{Time \& Light}}&\multicolumn{3}{c}{\textbf{Complex}}&\multicolumn{3}{c}{\textbf{Overall}}\\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19}\cmidrule(lr){20-22}
 Methods / Metrics
&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$&$\text{SRCC}_q$$\uparrow$&$\text{SRCC}_c$$\uparrow$&Acc$\uparrow$\\
    \midrule
     LLaVA-1.5(7B)~\cite{liu2024improved}& 0.3888  & 0.2547 & 0.7361 & 0.3088  & 0.4496 & 0.8012 & 0.4013 & 0.3751 & 0.6563 & 0.3953  & 0.5043 & 0.6843 & 0.3962 & 0.4129 & 0.7306 & 0.3363 & 0.4713 & 0.6629 & 0.3372 & 0.3887 & 0.7099 \\
    LLaVA-NeXT(8B)~\cite{liu2024llavanext}& 0.5342 & 0.2838  & 0.7052 & 0.5222 & 0.3131 & 0.8474 & 0.4745 & 0.4378 & 0.6465 & 0.5791 & 0.5684 & 0.6898 & 0.5039 & 0.4482  & 0.7054 & 0.4025 & 0.4127 & 0.5966 & 0.4333 & 0.4568 & 0.7067\\
    mPLUG-Owl3(7B)~\cite{ye2024mplug}& 0.4482 & 0.3993  & 0.7134 & 0.4576 & 0.3692 & 0.8032 & 0.0770 & 0.3402 & 0.6797 & 0.3537 & 0.4929 & 0.6679 & 0.3850 & 0.5390  & 0.6919 & 0.4022 & 0.5169 & 0.6465 & 0.3918 & 0.4744 & 0.7272 \\ 
   MiniCPM-V2.6(8B)~\cite{yao2024minicpm} & 0.4067 & 0.4041  & 0.7608 & 0.3821 & 0.4675 & 0.6165 & 0.3225 & 0.5104 & 0.7070 & 0.4746 & 0.6252 & 0.7153 & 0.4509 & 0.4639  & 0.6570 & 0.3328 & 0.5378 & 0.6614 & 0.3733 & 0.5916 & 0.7343\\
    Qwen2-VL(7B)~\cite{Qwen2-VL} & 0.5179 & 0.4879  & 0.7711 & 0.5896 & 0.5401 & 0.7972 & 0.4921 & 0.5768 & 0.6914 & 0.3851 & 0.5814 & 0.6788 & 0.5172 & 0.5433  & 0.6744 & 0.3502 & 0.6046 & 0.6222 & 0.3760 & 0.5899 & 0.7263\\
     Qwen2.5-VL(7B)~\cite{Qwen2.5-VL}& 0.5372  & 0.4566 & 0.7608 & 0.5620  & 0.4955 & 0.7048 & 0.6258 & 0.5486 & 0.7207 & 0.5984  & 0.6021 & 0.7263 & 0.5562 & 0.5039 & 0.6667 & 0.5487 & 0.6845 & 0.7470 & 0.5276 & 0.6401 & 0.7620\\
    Llama3.2-Vision(11B)~\cite{meta2024llama}
    &0.3114&0.1459&0.7301&0.2353&0.1404&0.6638&0.2741&0.0869&0.7128&0.2329&0.2267 &0.7035&0.3698&0.1299&0.6151&0.2842&0.1546&0.6086&0.2928&0.2598&0.7082\\
    Deepseekvl~\cite{lu2024deepseekvl}
    &0.3566&0.2277&0.7010&0.3553&0.2330&0.7666&0.2933&0.1772&0.6523&0.3113&0.5018&0.7007&0.3997&0.2524&0.6783&0.2054&0.3252&0.5675&0.2611&0.2356&0.7068 \\ 
    DeepseekVL2 (1B))~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.2001 &0.0838 &0.3052 &0.1747 &0.0126 &0.1687 &0.1683 &0.0394 & 0.4121 &0.1722 &0.0214 &0.3978 &0.1789 &0.0003 &0.3391 &0.0476 &0.0154 &0.6215 &0.1245 &0.0315 &0.4265\\
    DeepseekVL2 (2B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&0.2916 &0.0569 &0.4371 &0.2757 &0.1169 &0.2349 &0.3585 &0.0913 &0.5117 &0.2294 &0.1188 &0.5109 &0.4237 &0.0011 &0.5271 &0.2140 &0.0226 &0.5353 & 0.2577 & 0.0404 & 0.4921\\
  CogAgent(18B)~\cite{hong2024cogagentvisuallanguagemodel}& 0.3487 & 0.3081  & 0.7093 & 0.4351 & 0.3117 & 0.7932 & 0.4881 & 0.3656 & 0.6816 & 0.3953 & 0.3852 & 0.6223 & 0.4282 & 0.3137  & 0.6725 & 0.4128 & 0.2800 & 0.4804 & 0.3861 & 0.3575 & 0.6749 \\
  InternVL2(8B)~\cite{wang2024mpo}& 0.1341 & 0.4399  & 0.6825 & 0.2283 & 0.5327 & 0.7831 & 0.3015 & 0.3548 & 0.7031 & 0.2657 & 0.5622 & 0.7318 & 0.1645 & 0.3668  & 0.5833 & 0.1378 & 0.5257 & 0.6714 & 0.1492 & 0.5713 & 0.7198\\
    InternVL2.5(8B)~\cite{chen2024expanding}& 0.3068  & 0.3592 & 0.7031 & 0.3154  & 0.4264 & 0.7851 & 0.3009 & 0.4898 & 0.6660 & 0.3474  & 0.4890 & 0.7135 & 0.3329 & 0.3729 & 0.5640 & 0.2281 & 0.5904 & 0.6080 & 0.2597 & 0.5511 & 0.7006 \\
   InternLM-XComposer(7B)~\cite{internlmxcomposer}& 0.4482 & 0.2272  & 0.7134 & 0.4576 & 0.2054 & 0.8032 & 0.0770 & 0.1129 & 0.6797 & 0.3537 & 0.1877 & 0.6679 & 0.3850 & -0.0196 & 0.6919 & 0.4022 & 0.1697 & 0.6465 & 0.3918 & 0.1728 & 0.7272\\
    Llava-Onevision(0.5B)~\cite{li2024llava}& 0.1199  & 0.1168 & 0.7361 & 0.1515 & 0.2728 & 0.2972 & 0.3006 & 0.3131 & 0.5957 & 0.0140  & 0.4547 & 0.4288 & 0.2070 & 0.2153 & 0.3857 & 0.0379 & 0.1377 & 0.6593 & 0.1192 & 0.2494 & 0.6175\\
   \hline
      *DeepseekVL2 (1B)~\cite{wu2024deepseekvl2mixtureofexpertsvisionlanguagemodels}&\bf\blue{0.7711} & 0.6704&0.8392 &\bf\blue{0.8152} &0.6777 & 0.8976 &0.8370 &\bf\blue{0.6892}& 0.7715&\bf\blue{0.7670} & \bf\blue{0.7636} & 0.8175 &\bf\blue{0.7713} & 0.6659 & 0.8256&\bf\blue{0.7689}  &0.7780 &0.8368 &\bf\blue{0.7899} &0.7817& 0.8494\\
      *Qwen2.5-VL (8B)~\cite{Qwen2.5-VL}& 0.7117  & \bf\blue{0.7815} & \bf\blue{0.8557} & 0.7339  & \bf\blue{0.7134} & \bf\blue{0.9037} & 0.7596& 0.6484 & \bf\blue{0.8218} & 0.5942  & 0.7356 & \bf\blue{0.8796} & 0.7069& \bf\blue{0.7175} & \bf\blue{0.8272} & 0.6675 & \bf\blue{0.8111} & \bf\blue{0.8915} & 0.6990 & \bf\blue{0.8008} & \bf\blue{0.8719}\\
    *Llama3.2-Vision (11B)~\cite{meta2024llama}&0.7184 & 0.2582& 0.8144& 0.7585& 0.6577& 0.8795&\bf\blue{0.8374} &0.5978&0.7734&0.7230 & 0.6238& 0.7956&0.7448 & 0.6526& 0.8217&0.7135 & 0.5317&0.7591&0.7556& 0.6403&0.7807 \\
   %\hdashline
   \rowcolor{gray!20} \textbf{LMM4LMM (Ours)} &\bf\red{0.8702}&\bf{\red{0.8141}}&\bf\red{0.8495}&\bf\red{0.8852}&\bf\red{0.8135}&\bf\red{0.9046}&\bf\red{0.9488}&\bf\red{0.9063}&\bf\red{0.8242}&\bf\red{0.8859}&\bf\red{0.8822}&\bf\red{0.8850}&\bf\red{0.8783}&\bf\red{0.82291}&\bf\red{0.8295}&\bf\red{0.8768}&\bf\red{0.9008}&\bf\red{0.8924}&\bf\red{0.8863}&\bf\red{0.8950}&\bf\red{0.8794}\\
   %\textit{Improvement}&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&-\\
    \bottomrule[1pt]
  \end{tabular}}
  \label{lmm}
  % \vspace{-1em}
\end{table*}

==> tabels/model2.tex <==
\begin{table*}[tbph]
\vspace{-1mm}
% \setlength{\belowcaptionskip}{-0.01cm}
\centering
% \belowrulesep=0pt
% \aboverulesep=0pt
\renewcommand\arraystretch{0.6}
\caption{
}
\vspace{-6mm}
   \resizebox{\linewidth}{!}{\begin{tabular}{l||cc:cc:cc|cc:cc:cc|cc:cc:cc|c:c:c}
    \toprule[1pt]
    Dimension  &\multicolumn{6}{c|}{\textbf{Quality MOS}}&\multicolumn{6}{c|}{\textbf{Correspondence MOS}}&\multicolumn{6}{c|}{\textbf{Question Answering Accuracy}}&\multicolumn{3}{c}{\textbf{Overall Rank}}\\
  \cmidrule(lr){2-7}  \cmidrule(lr){8-13} \cmidrule(lr){14-19} \cmidrule(lr){20-22}
 Models
&$\text{Human}_s$$\uparrow$&$\text{Human}_r$$\uparrow$&$\text{Ours}_s$$\uparrow$&$\text{Ours}_r$$\uparrow$&$\text{Q-Align}_s$$\uparrow$&$\text{Q-Align}_r$$\uparrow$&$\text{Human}_s$$\uparrow$&$\text{Human}_r$$\uparrow$&$\text{Ours}_s$$\uparrow$&$\text{Ours}_r$$\uparrow$&$\text{FGA}_s$$\uparrow$&$\text{FGA}_r$$\uparrow$&$\text{Human}_s$$\uparrow$&$\text{Human}_r$$\uparrow$&$\text{Ours}_s$$\uparrow$&$\text{Ours}_r$$\uparrow$&$\text{Qwen2.5}_s$$\uparrow$&$\text{Qwen2.5}_r$$\uparrow$&$\text{Human}_r$$\uparrow$&$\text{Ours}_r$$\uparrow$&$\text{Other}_r$$\uparrow$\\
    \midrule
    ali\_flux\_schnell~\cite{niqe} & 60.63  & 4 & 61.51 & 3  & 92.69 & 6 & 58.10 & 2 & 58.38 & 3  & 3.50 & 4 & 80.29 & 2 & 78.64 &3 & 71.62 & 4& 1 & 1 & 4\\
    sd3\_5\_large~\cite{qac} & 59.50 & 5  & 59.77& 7 & 88.78 & 10 & 58.35 & 1 & 59.04 & 1 & 3.58 & 1 & 81.43  & 1 & 82.18 & 1 & 76.86 & 2 & 2 & 3&5  \\
    playground~\cite{hosa} & 61.64 & 1  & 62.89 & 1 & 96.40 & 1 & 56.06 & 5 & 57.46 & 5 & 3.56 & 2 & 73.86 & 5  & 74.13 & 5 & 68.16 & 7 & 3 & 2 & 1 \\ 
   Infinity~\cite{}& 60.86 & 3  & 61.50 & 4 & 95.73 & 2 & 57.43 & 4 & 58.17 & 4 & 3.45 & 5 & 78.10 & 4  & 77.32 & 4 & 67.68 & 8 & 4 & 4 & 3\\
    DALLE3~\cite{korhonen2019two} & 59.35 & 6  & 60.27 & 6 & 94.72 & 4 & 57.97 & 3 & 58.38 & 2 & 3.52 & 3 & 80.24 & 3  & 79.15 & 2 & 80.05 & 1 & 5 & 5 & 2\\
    Kolors~\cite{korhonen2019two}& 61.14  & 2 & 62.29 & 2  & 95.70 & 3 & 53.53 & 9 & 55.07 & 8  & 3.24 & 11 & 65.05 & 10 & 69.00 & 9 & 61.99 & 14 & 6 & 6 & 6\\
    omnigen~\cite{tu2021ugc}
    &59.12&7&60.47&5&91.04&8&55.81&6&57.00&6&3.38 &7&73.29&6&72.75&6&65.45&9&7&7&8\\
    PixArt-sigma~\cite{tu2021rapique}
    &57.43&9&59.19&8&91.11&7&54.72 &7&56.07 &7&3.39 &6&70.71 &8&70.49 &8&64.87 &11&8&8&7 \\
    Show-o~\cite{li2019quality}&52.31 &12 &52.74 &12 &83.61 &13 &54.21 &8&54.54 &9&3.38 &8&71.71 &7&71.74 &7&71.74 &3&9&9&9\\
    sdxl\_base\_1~\cite{li2019quality}&53.50 &11 &54.45 &11 &87.28 &12 &52.23 &11&53.51 &11&3.29 &9&63.67 &11&65.82 &12&64.05 &13&10&10&11\\
  EMU3~\cite{chen2021learning}& 54.29 & 10  & 54.86 & 10 & 87.58 & 11 & 50.97 &12&52.61 &14&3.12 &14&59.90 &13&61.56 &15&57.67 &18&11&12&15 \\
  NOVA~\cite{}& 50.69 & 14  & 51.35 & 14 & 79.61 & 16 & 52.73 &10&52.77 &13&3.29 &10&68.19 &9&66.89 &10&68.69 &6&12&14&13\\
   Kandinsky-3~\cite{sun2022deep}& 58.21  & 8 & 58.74 & 9  & 93.58 & 5 & 48.37 &17&51.60 &15&2.84 &18&50.14 &17&57.60 &16&52.45 &20&13&13&12 \\
   seed-xi~\cite{wu2022fast}& 50.73 & 13  & 51.49 & 13 & 79.74 & 15 & 50.96 &13&53.93 &10&3.18 &12&61.43 &12&66.28 &11&64.91 &10&14&11&14\\
   LaVi-Bridge~\cite{wu2023exploring}& 50.56  & 15 & 51.16 & 15  & 66.27 & 18 & 50.19 &15&51.01 &16&3.08 &16&59.10 &15&62.40 &13&55.61 &19&15&15&19\\
   hart&49.80&16&49.85&17&88.87 & 9&50.30 &14&53.04 &12&3.14 &13&59.29 &14&61.99 &14&59.81 &15&16&16&10\\
   ELLA&44.61&19&45.17&19&57.68&19&49.07 &16&50.14 &18&3.10 &15&54.90 &16&56.71 &17&64.71 &12&17&18&17\\
   sd\_v2-1&47.68&18&49.23&18&75.27&17&47.96 &18&50.41 &17&3.02 &17&48.86 &18&54.39 &18&58.19 &17&18&17&18\\
   LLMGA&48.67&17&50.54&16&81.63&14&43.43 &21&46.21 &20&2.59 &21&37.67 &20&43.58 &20&40.04 &24&19&19&20\\
   Janus&36.98&20&37.34&20&41.82&20&45.94 &19&47.16 &19&2.82 &19&42.95 &19&48.67 &19&68.77 &5&20&20&16\\
   vila-u&33.80&22&33.18&22&19.54&22&43.47 &20&44.32 &21&2.61 &20&35.24 &21&35.85 &21&58.78 &16&21&21&21\\
   i-Code-V3&34.70&21&35.14&21&20.76&21&39.80 &22&40.49 &22&2.41 &22&25.00 &22&30.98 &22&41.31 &22&22&22&22\\
   LlamaGen\_256&29.96&23&30.74&23&12.18&23&37.73 &23&39.09 &23&2.31 &23&21.19 &23&22.88 &23&47.30 &21&23&23&23\\
   LWM&28.88&24&29.26&24&11.54&24&35.46 &24&36.52 &24&2.09 &24&15.48 &24&15.88 &24&40.04 &23&24&24&24\\
   \hline
   SRCC to human & - & - & 0.7723 & 0.9939\\
   %\hdashline
   % \rowcolor{gray!20} \textbf{AIGIQA (Ours)} &\bf\red{0.8497}&\bf{\red{0.7989}}&\bf\red{0.8951}&\bf\red{0.8608}&\bf\red{0.8989}&\bf\red{0.8933}&\bf\red{0.8681}&\bf\red{0.8667}&\bf\red{0.8750}&\bf\red{0.8597}&\bf\red{0.8260}&\bf\red{0.8954}&\bf\red{0.8512}&\bf\red{0.8411}&\bf\red{0.8876}&\bf\red{0.8627}&\bf\red{0.8167}&\bf\red{0.8184}&\bf\red{0.8053}&\bf\red{0.8522}&\bf\red{0.8705}\\
    \bottomrule[1pt]
  \end{tabular}}

 \vspace{-2mm}
\end{table*}
